Electromagnetic response of dense quark matter around color-superconducting phase transition and QCD critical point

We explore how the electric conductivity and associated relaxation time are modified near the QCD critical point and the phase transition to a color superconducting phase using the two-flavor Nambu-Jona-Lasinio model with finite current quark masses. We give a comprehensive account of the nature of the soft modes associated with these phase transitions and how they affect the photon self-energy when the system approaches these phase transitions in a combined way with an emphasis on the common and different aspects in the two transitions. The formalism developed for describing the paraconductivity in metallic superconductors is used for the analysis of the photon self-energy. We show that the transport coefficients calculated from the self-energy show anomalous enhancements in both cases with different critical exponents for the individual transitions. We briefly discuss the possibility of detecting the enhancements in the relativistic heavy-ion collisions in the present and future facilities.

==> Chap_TransportCoeff.tex <==
\chapter{Transport coefficients}
\label{chap:TransportCoeff}

In this chapter, we investigate the effect of the soft modes on the transport coefficients, 
electric conductivity $\sigma$ and associated relaxation time $\tau_\sigma$,
through the analysis of the photon self-energy that has been constructed in Chap.~\ref{chap:PI}.
This study is based on Ref.~\cite{Nishimura:2024}.

To start the analysis of the transport coefficients, 
we define the spectral density at zero momentum 
using the retarded function of the photon self-energy~\eqref{eq:PI_tot} 
by the manner described in Sec.~\ref{sec:DPR-Coeff}:
\begin{align}
\rho(\omega) = g_{\mu\nu} {\rm Im}\Pi^{R \mu\nu}(\bm{0}, \omega)
= -\sum_{i=1,2,3} {\rm Im}\Pi^{R ii}(\bm{0}, \omega) .
\label{eq:rho_def}
\end{align}
Since the Ward identity for the photon self-energy~\eqref{eq:PI-WT} is satisfied,
the coefficients $\sigma$ and $\tau_\sigma$ can be read using Eq.~\eqref{eq:sigma-tau} as follows 
\begin{align}
\sigma 
= \frac{1}{3} \frac{\partial \rho(\omega)}{\partial \omega} \bigg|_{\omega=0} ~~,
\hspace{0.5cm} 
\tau_\sigma 
= \sqrt{ -\frac{1}{3!} \frac{\partial^3 \rho(\omega)}{\partial^3 \omega} \bigg|_{\omega=0}
~~\Big/~~ \frac{\partial \rho(\omega)}{\partial \omega} \bigg|_{\omega=0} } ~~.
\label{eq:sigma-tau}
\end{align}
Eq.~\eqref{eq:PI_tot} consists of the three contributions, 
and then the spectral density~\eqref{eq:rho_def} is decomposed as
\begin{align}
\rho(\omega) &= \rho_{\rm free}(\omega) + \rho_D(\omega) + \rho_S(\omega)
\end{align}
with
\begin{align}
\rho_{\rm free}(\omega) =& -\sum_i {\rm Im}\Pi_{\rm free}^{R ii}(\bm{0},\omega),
\label{eq:rho_free} \\
\rho_\gamma(\omega) =& -\sum_i {\rm Im}\Pi_\gamma^{R ii}(\bm{0}, \omega)
\quad \text{for} \quad \gamma=D,S .
\label{eq:rho_D-S}
\end{align}


In our formalism, the photon self-energy with the soft modes consists of the AL, MT, and DOS terms.
Of these terms, however, the spatial components of the MT and DOS terms cancel as in 
Eqs.~\eqref{eq:MT-DOS-cancel_D} and~\eqref{eq:MT-DOS-cancel_S}.
Thereby, the contributions of the soft modes $\rho_\gamma(\omega)$ is given by only the AL term,
and then $\partial^n \rho_\gamma(\omega) / \partial^n \omega |_{\omega=0}$ for $n=1,3$
are calculated with Eqs.~\eqref{eq:ImAL-explicit_D} and~\eqref{eq:ImAL-explicit_S} as follows
\begin{itemize}
\item the LE approximation
\begin{align}
\hspace{-0.7cm}
\frac{\partial^n \rho_D(\omega)}{\partial^n \omega} \bigg|_{\omega=0}
&= ~2\bar{N}_\gamma
\int \frac{d^3q}{(2\pi)^3} ~\bigg( \frac{\partial A_\gamma(\bm{q})}{\partial|\bm{q}|} \bigg)^2 
\int d\omega' \coth\frac{\omega'}{2T} 
\nonumber \\
&\hspace{3.5cm} \times
~{\rm Im}\Xi^R_\gamma(\bm{q}, \omega')
~\frac{\partial^n}{\partial^n \omega'} {\rm Im}\Xi_\gamma^R(\bm{q}, \omega') ,
\label{eq:rho_gamma_LE}
\end{align}
%
%
\\[-1.8cm]
%
%
\item the TDGL approximation
\begin{align}
\hspace{-0.7cm}
\frac{\partial^n \rho_D(\omega)}{\partial^n \omega} \bigg|_{\omega=0}
&= ~2\bar{N}_\gamma
\int \frac{d^3q}{(2\pi)^3} ~\big( 2b_\gamma\bm{q} \big)^2 
\int d\omega' \coth\frac{\omega'}{2T} 
\nonumber \\ 
&\hspace{3.5cm} \times
~{\rm Im}\Xi^R_\gamma(\bm{q}, \omega')
~\frac{\partial^n}{\partial^n \omega'} {\rm Im}\Xi_\gamma^R(\bm{q}, \omega') .
\label{eq:rho_gamma_TDGL}
\end{align}
\end{itemize}
To obtain Eq.~\eqref{eq:rho_gamma_LE}, 
$A_\gamma^{(1)}(\bm{q}+\bm{k}, \bm{q}) |_{\bm{k}=\bm{0}}
= \partial A_\gamma / \partial |\bm{q}|$ has been used, 
where $A_\gamma^{(1)}(\bm{q}_1, \bm{q}_2)$ has been defined 
by Eqs.~\eqref{eq:A-derivative_D} and~\eqref{eq:A-derivative_S} 
for $\gamma=D$ and $S$, respectively.
% In Eqs.~\eqref{eq:rho_gamma_LE} and~\eqref{eq:rho_gamma_TDGL}, 
Also, the overall coefficient $N_\gamma$ is 
\begin{align}
\bar{N}_D = 3e_\Delta^2, 
\hspace{0.5cm}
\bar{N}_S = e_u^2+e_d^2.
\label{eq:overall-coeff}
\end{align}
The integrand of $\partial^n \rho_\gamma(\omega) / \partial^n \omega |_{\omega=0}$ for $n=1,3$ 
becomes divergent at $(\bm{q}, \omega') = (\bm{0}, 0)$ as the system approaches the critical points,
which is due to the property of the soft modes that have been described in Chap.~\ref{chap:SoftMode}.
Then, this leads to the divergence of $\sigma$ and $\tau_\sigma$ at the 2SC-PT and QCD-CP.
Therefore, near the 2SC-PT, the contribution from $\rho_D(\omega)$ is dominates 
over the one from $\rho_S(\omega)$ and the behavior of $\sigma$ and $\tau_\sigma$ 
is described only by $\rho_D(\omega)$, and vice versa.
In this thesis, we calculate the transport coefficients 
from $\rho_D(\omega)$ and $\rho_S(\omega)$ separately near the 2SC-PT and QCD-CP, respectively, 



On the other hand, $\rho_{\rm free}(\omega)$ does not contribute to $\sigma$ and $\tau_\sigma$ 
since $\rho_{\rm free}(\omega) = 0$ for $|\omega| < 2M$ and $M$ is finite.
From Eq.~\eqref{eq:ImPI_free-massive_explicit}, its density is given by
\begin{align}
\rho_{\rm free}(\omega) = \frac{N_c(e_u^2+e_d^2)}{4\pi} (\omega^2+2M^2)
\sqrt{ \frac{\omega^2-4M^2}{\omega^2} }
\sum_{s=\pm} \tanh \frac{\omega-2s\mu}{4T} ~\theta(|\omega|-2M) ,
\label{eq:rho_free_massive}
\end{align}
and then all its $\omega$ derivatives vanish at $\omega=0$.
Even in the massless case, $\rho_{\rm free}(\omega)$ cannot give a finite contribution to $\sigma$.
Taking the limit $\omega \to 0$ at $M=0$, Eq.~\eqref{eq:rho_free_massive} becomes
\begin{align}
\rho_{\rm free}(\omega)|_{M=0}
&= \frac{N_c(e_u^2+e_d^2)}{8\pi} \cosh^{-2} 
\frac{\mu}{2T} ~\frac{\omega^3}{T}
+ \mathcal{O}(\omega^5) .
\label{eq:rho_free_massless}
\end{align}
From this, $\partial\rho_{\rm free}(\omega) / \partial\omega |_{\omega=0} = 0$ can be checked.
Also, the contribution of $\rho_{\rm free}(\omega)$ to $\tau_\sigma$ is neglected
since$\partial^3\rho_\gamma(\omega) / \partial^3\omega \gg
\partial^3\rho_{\rm free}(\omega) / \partial^3\omega$ around the 2SC-PT and QCD-CP

 






% In Sec.~\ref{sec:analytical}, we investigate the behavior of the coefficients
% due to the soft modes in the critical region through the analytical calculations
% of Eq.~\eqref{eq:rho_gamma_TDGL} with the TDGL approximation and some simplifications
% and show the divergences of their transport coefficients 
% at the critical points and their critical exponents.
% Then, we show the numerical results in Sec.~\ref{sec:numerical}.












%----------------------------------------------------------------------------------------
%	SECTION 
%----------------------------------------------------------------------------------------
\section{Analytical results}
\label{sec:analytical}

Let us investigate the limiting behaviors of the transport coefficients
$\sigma$ and $\tau_\sigma$ as the system approaches the 2SC-PT or QCD-CP 
with the TDGL approximation~\eqref{eq:rho_gamma_TDGL}
that allows us to calculate the critical exponents of those coefficients analytically.

Firstly, we consider the case of 2SC-PT. 
Since the strength from the soft modes is concentrated 
around the origin of energy/momentum plane near the 2SC-PT, 
the dominant contribution to $\sigma$ and $\tau_\sigma$ from the soft modes exists there.
Then, in Eq.~\eqref{eq:rho_gamma_TDGL}, one can carry out the following replacement 
\begin{align}
\coth ~\frac{\omega'}{2T} ~~\to~~ \frac{2T}{\omega'} .
\label{eq:coth}
\end{align}
Also, since the integrand of $\partial^n \rho_D(\omega) / \partial^n \omega |_{\omega=0}$
converges in the $|\omega'| \to \infty$ and $|\bm{q}| \to \infty$ limit,
the integration range can be deformed as
\begin{align}
\int \frac{d^3q}{(2\pi)^3} \int d\omega'
= \int^{2\sqrt{\mu^2-M^2}}_0 q^4 dq 
\int^{\bar\Lambda}_{\lambda(q,0)-2\mu} d\omega'
~~\to~~ \int^{\infty}_0 q^4 dq \int^{+\infty}_{-\infty} d\omega'.
\label{eq:integral_rhoD}
\end{align}
Here, the first equality is due to the limitation of approximation 
for ${\rm Im}\Xi_D^R(\bm{q}, \omega')$ as described in Sec.~\ref{sec:SoftMode_D}.
By these simplifications % ~\eqref{eq:coth} and~\eqref{eq:integral_rhoD},
we can calculate Eq.~\eqref{eq:rho_gamma_TDGL} for $\gamma=D$ analytically as follows
\begin{align}
\frac{\partial \rho_D(\omega)}{\partial \omega} \bigg|_{\omega=0}
=&~-\frac{9 e_\Delta^2 T}{16 \pi} 
\frac{|c_D|^2}{{\rm Im} c_D}
\frac{1}{a_D^{1/2} b_D^{1/2}} ,
\label{eq:deff-rho-1_D} \\
\frac{\partial^3 \rho_D(\omega)}{\partial^3 \omega} \bigg|_{\omega=0}
=&~\frac{27 e_\Delta^2 T}{512 \pi}
\frac{|c_D|^6}{({\rm Im}c_D)^3}
\frac{1}{a_D^{5/2} b_D^{1/2}} ,
\label{eq:deff-rho-3_D}
\end{align}
where $\partial \rho_D(\omega) / \partial \omega |_{\omega=0}$
and $\partial^3 \rho_D(\omega) / \partial^3 \omega |_{\omega=0}$
are positive and negative numbers, respectively, because of ${\rm Im}c_D < 0$.
These detailed calculations are in Appendix~\ref{appendix:Exponents}.



Inserting Eqs.~\eqref{eq:deff-rho-1_D} and~\eqref{eq:deff-rho-3_D} into Eq.~\eqref{eq:sigma-tau} 
and using Eq.~\eqref{eq:coeff-simlifiedTDGL1}, we obtain 
\begin{align}
\sigma \sim T \frac{|c_D|}{a_D^{1/2} b_D^{1/2}} \sim \frac{T}{\epsilon^{1/2}} ,
\qquad
\tau_\sigma \sim \sqrt{\frac{|c_D|^2}{a_D^2}} \sim \frac{1}{T \epsilon} .
\label{eq:coefficients-behavior_D}
\end{align}
This result shows that both coefficients diverge at $T = T_c$ and 
the critical exponents of $\sigma$ and $\tau_\sigma$ are $-1/2$ and $-1$, respectively.
Regarding conductivity, the exponent is the same as the one 
in the case of the ultra-clean case of the three-dimensional metal~\cite{Larkin:book},
where only the AL term can give a critical contribution 
owing to the cancellation of the MT and DOS terms as well.

Equation~\eqref{eq:coefficients-behavior_D} also tells us that 
the magnitude of $\sigma$ and $\tau_\sigma$ does not depend on either $\mu$ or $G_D$ 
explicitly within the approximation~\eqref{eq:coeff-simlifiedTDGL2}.
This suggests that $\sigma$ and $\tau_\sigma$ are insensitive to $\mu$ around the 2SC-PT.
These analytic results will be checked numerically in Sec.~\ref{sec:numerical} with the LE approximation.
Using $\xi_D$ and $\tau_{\rm D}$ that are introduced in Eq.~\eqref{eq:xi-tau}, 
Eq.~\eqref{eq:coefficients-behavior_D} is rewritten as
\begin{align}
\sigma \sim T \frac{\tau_{\rm D}}{\xi_D} ,
\qquad
\tau_\sigma \sim \tau_{\rm D} .
\end{align}
From this, it is found that the typical time scale of the relaxation to the Ohm's law
is given by the one of the damping of the soft modes.


Next, we consider the case of the QCD-CP.
In the same manner as the case of the 2SC-PT, the replacement of Eq.~\eqref{eq:coth} 
in the TDGL approximation~\eqref{eq:rho_gamma_TDGL} can be applied for the case of $\gamma=S$.
In this case, since the soft mode is restricted to the space-like region 
($|\omega + 2\mu| < \bar{k}(|\bm{k}|, \bar\Lambda)$) as described in Sec.~\ref{sec:SoftMode_S},
we deform the integration region of $\partial^n \rho_D(\omega) / \partial^n \omega |_{\omega=0}$ as
\begin{align}
\int \frac{d^3q}{(2\pi)^3} \int d\omega'
= \int^{\bar\Lambda}_0 q^4 dq 
\int^{+\bar{k}(|\bm{k}|, \bar\Lambda))}_{-\bar{k}(|\bm{k}|, \bar\Lambda))} d\omega'
~~\to~~ \int^{\infty}_0 q^4 dq \int^{+q}_{-q} d\omega'.
\label{eq:integral_rhoS}
\end{align}
Finally, we then obtain
\begin{align}
\frac{\partial \rho_S (\omega)}{\partial \omega} \bigg|_{\omega=0}
&=~\frac{(e_u^2+e_d^2) T}{2 \pi^3} 
\frac{{\rm Im}c_S}{a_S} ~{\rm tan}^{-1} \frac{{\rm Im}c_S}{a_S},
\label{eq:deff-rho-1_S} \\
\frac{\partial^3 \rho_S (\omega)}{\partial^3 \omega} \bigg|_{\omega=0}
&=~\frac{(e_u^2+e_d^2) T}{2 \pi^3} 
\frac{3 b_S ({\rm Im}c_S)^3}{4 a_S^4} ~{\rm tan}^{-1} \frac{{\rm Im}c_S}{a_S}.
\label{eq:deff-rho-3_S}
\end{align}
These detailed calculations are also given in Chap.~\ref{appendix:Exponents}.
As seen in Eq.~\eqref{eq:aS}, the exponent of $a_S$ with respect to 
$\epsilon_{\rm CP}$ depends on the direction to approach the CP,
while $b_S$ and $c_S$ are insensitive to $\epsilon_{\rm CP}$.
Inserting Eqs.~\eqref{eq:deff-rho-1_S} and~\eqref{eq:deff-rho-3_S} into Eq.~\eqref{eq:sigma-tau} 
and using Eq.~\eqref{eq:aS}, one thus can find the exponents of the divergences as follows
\begin{align}
\sigma \sim \frac{1}{a_S} &\sim
\begin{cases}
~\epsilon_{\rm CP}^{-1} &\text{parallel to the first-order line,} \\
~\epsilon_{\rm CP}^{-2/3} & \text{otherwise,} 
\end{cases}
\label{eq:sigma-behavior_S} \\
\tau_\sigma \sim \frac{1}{a_S^{3/2}} &\sim
\begin{cases}
~\epsilon_{\rm CP}^{-3/2} & \text{parallel to the first-order line,} \\
~\epsilon_{\rm CP}^{-1} & \text{otherwise.} 
\end{cases}
\label{eq:tau-behavior_S}
\end{align}
Unlike in the case of the 2SC-PT, the critical exponents due to the QCD-CP soft modes
depend on the way to approach the critical point.

Before closing this subsection, several remarks are in order.
First, as mentioned in Sec.~\ref{sec:PI_D}, the above results 
are obtained in the linear approximation for the soft modes. 
The critical exponent thus corresponds to the mean-field ones. 
The non-linear effects will be negligible near the 2SC-PT and QCD-CP, 
which will alter the critical exponents to the values determined by the universality class. 
We, however, emphasize that our analysis gives the values of 
$\sigma$ and $\tau_\sigma$ up to the absolute value, 
while the universal argument is not capable of constraining them.
Second, let us discuss the origin of the different critical exponents.
The dependencies of $\sigma$ and $\tau_\sigma$ on the TDGL coefficient 
$a_\gamma$ are different from each other, which is caused by the differences 
in the momentum dependence of the soft mode propagators $\Xi^R_\gamma(\bm{k}, \omega)$.
Additionally, the exponents of $a_D$ and $a_S$ differ 
as shown in Eqs.~\eqref{eq:coeff-simlifiedTDGL1} and~\eqref{eq:aS}.
These two differences in the properties of the soft modes 
cause the various exponents of the transport coefficients.
It is fascinating that the different exponents can be obtained 
even though the effects of soft modes are taken into account at the RPA level.










%----------------------------------------------------------------------------------------
%	SECTION 
%----------------------------------------------------------------------------------------
\section{Numerical results}
\label{sec:numerical}


In this section, we study the behavior of $\sigma$ and $\tau_\sigma$ numerically 
with the LE approximation~\eqref{eq:rho_gamma_LE}
and TDGL approximations~\eqref{eq:rho_gamma_TDGL}. 

\begin{figure*}[t]
\centering
\hspace{-1.1cm}
\includegraphics[keepaspectratio, scale=0.76]{Figures/sigma_2SCPT.pdf}
\\[0.2cm]
\centering
\hspace{-1.1cm}
\includegraphics[keepaspectratio, scale=0.76]{Figures/tau_2SCPT.pdf}
\\
\caption
{Electric conductivity and associated relaxation time due to the soft modes 
of the 2SC-PT at several values of $\mu$ and $G_D$.
The thick red and thin blue lines are calculated 
by the LE and the TDGL approximation, respectively.
The dotted line in each panel represents the critical exponent
given in Eq.~\eqref{eq:coefficients-behavior_D}.
In the left panels, the lines are plotted 
at $\mu = 350$, $400$, $500~{\rm MeV}$ with $G_D= 0.7 G_S$,
while the right panels, the lines are plotted 
with $G_D = 0.70$, $0.65$, and $0.60 G_S$ at $\mu = 350 {\rm MeV}$.}
\label{fig:SigmaTau_D}
\end{figure*}




First, let us see the behavior of $\sigma$ and $\tau_\sigma$ near the 2SC-PT.
Figure~\ref{fig:SigmaTau_D} shows $\sigma/T$ (upper panels) and $\tau_\sigma T$ (lower panels) 
that are obtained from $\rho_D(\omega)$. These are plotted as functions of $\epsilon=(T-T_c)/T_c$.
The left panels show the results for $\mu = 350$, $400$, $500~{\rm MeV}$ with fixed $G_D = 0.7 G_S$, 
while the results on the right panels are plotted with several values of $G_D$ at fixed $\mu=350~{\rm MeV}$.
The thick-red (thin-blue) lines represent the results obtained with the LE (TDGL) approximation.
It is found that $\sigma / T$ and $\tau_\sigma T$ grows as $\epsilon \to 0$.
One also sees that the LE and TDGL results converge to the same behavior in this limit, 
while their difference grows as $\epsilon$ becomes larger.
As explained in Sec.~\ref{sec:PI-vertex_D}, this is a reasonable result 
because the TDGL approximation is well justified only in the vicinity of $T_c$ 
where the strength of the soft modes is concentrated at the small energy-momentum region.
For large $\epsilon$, the TDGL result tends to underestimate the LE one. 
This result is mainly attributed to the behavior 
of the vertex function as discussed in Sec.~\ref{sec:PI-vertex_D}.
To check the critical exponents of $\sigma$ and $\tau_\sigma$, in Fig.~\ref{fig:SigmaTau_D} 
we show the slope of exponent in Eq.~\eqref{eq:coefficients-behavior_D} by the thin dotted lines.
One sees that the numerical results are in good agreement with these analytic results.
Another interesting feature found in the figure is that the numerical results 
on $\sigma/T$ and $\tau_\sigma T$ are insensitive to $\mu$ and $G_D$. 
This result is expected from Eq.~\eqref{eq:coefficients-behavior_D}.






\begin{figure*}[t]
\centering
\hspace{-1.3cm}
\includegraphics[keepaspectratio, scale=0.59]{Figures/sigma_QCDCP.pdf}
\\
\centering
\hspace{-1.3cm}
\includegraphics[keepaspectratio, scale=0.59]{Figures/tau_QCDCP.pdf}
\caption
{Electric conductivity and associated relaxation time due to the soft modes of the QCD-PT.
The red thick and blue thin lines are calculated 
by the LE and the TDGL approximation, respectively.
The upper and lower panels are the results of $\sigma / T$ and $\tau_\sigma T$, respectively.
The left panels are plotted along the crossover transition lines or first-order PT.
The middle and right panels are plotted along the $T$-direction at $\mu = \mu_{\rm CP}$ 
and along the $\mu$-direction at $T = T_{\rm CP}$, respectively.
The thin dotted line in each panel represents the exponents of divergence as 
in Eqs.~\eqref{eq:sigma-behavior_S} and~\eqref{eq:tau-behavior_S}.}
\label{fig:SigmaTau_S}
\end{figure*}

Next, we show the numerical results for the QCD-CP in Fig.~\ref{fig:SigmaTau_S}.
The upper and lower panels are the results of $\sigma / T$ and $\tau_\sigma T$ 
calculated from $\rho_S(\omega)$. These are plotted with respect to $\epsilon_{\rm CP}$.
In the left panels, $T$ and $\mu$ are varied along the line parallel 
to the first-order transition line passing through the CP,
where the results for $T<T_{\rm CP}$ are plotted 
for two coexisting phases on the first-order phase transition,
while the ones for $T>T_{\rm CP}$ is plotted along the crossover transition line.
In the middle panels, we set $\mu = \mu_{\rm CP}$, 
while, in the right panels, $T$ is fixed at $T_{\rm CP}$.
In these panels, the thick-red and thin-blue lines are the results obtained by
the LE and TDGL approximations, respectively,
while the thin-dotted black lines represent the exponents 
given in Eqs.~\eqref{eq:sigma-behavior_S} and~\eqref{eq:tau-behavior_S}.

The above figures show that the numerical results reproduce these critical behaviors near the QCD-CP.
In particular, near the critical point, the coefficients behave as in
the exponents expected in the previous section in all panels.
In the left panels, one finds that the magnitude of the results 
are different when $T$ and $\mu$ approach the critical point
along the first-order phase transition and crossover transition lines.
This difference is explained as follows.
The thermodynamic potential~\eqref{eq:omega_MFA} are expanded with respect to the chiral condensate
as in the Landau free energy~\eqref{eq:energy_L} near the QCD-CP.
In this case, the coefficient $a_S$ behaves as in Eq.~\eqref{eq:chi_h-zero} 
along the first-order phase transition and crossover transition.
The difference of the magnitude reflects the behavior of $a_S$.
Also, the results from the LE and TDGL approximations are consistent with each other around the critical point.
However, as $T$ and/or $\mu$ go away from the CP, they become to deviate.
This is because the vertex function of the TDGL approximation disagrees 
with the one of the LE approximation as shown in Fig.~\ref{fig:Gamma_S}.

\begin{figure}[t]
\centering
\hspace{0.1cm}
\includegraphics[keepaspectratio, scale=0.83]{Figures/Sigma3d.pdf}
\caption
{Contour maps of $\sigma / T$ in the $T$-$\mu$ plane 
around the CP with $G_D / G_S= 0.70$, $0.65$ and $0.60$.
The solid and dashed lines are the first-order and second-order phase transitions, respectively.}
\label{fig:Sigma3d}
\end{figure}

Here, we see the behavior of $\sigma / T$ including the effects 
of both 2SC-PT and QCD-CP soft modes on the phase diagram.
In Fig.~\ref{fig:Sigma3d}, we show the contour maps of $\sigma / T$ 
on the $T$--$\mu$ plane around the first-order transition line for three values of 
the diquark couplings at $G_D = 0.70G_S$, $0.65G_S$, and $0.60G_S$.
This figure is obtained by the LE approximations.
The solid and dashed lines show the first-order phase transition 
and the  second-order phase transition of the 2SC, respectively.
Since our formalism is not applicable to the 2SC phase where the diquark condensate 
has a nonzero expectation value $\Delta \ne 0$, this phase is left blank in the figure.
One finds that $\sigma / T$ is enhanced around the 2SC-PT and QCD-CP.
A significant enhancement due to the QCD-CP soft mode occurs 
along the critical line parallel to the first-order transition line.
For $G_D = 0.7G_S$, this enhancement is almost connected to the one due to the 2SC-PT soft modes. 
However, these two enhancements move away from each other 
since $T_c$ of the 2SC-PT is lowered as the value of $G_D$ decreases.
Since the electric conductivity is related to the low energy-momentum behavior 
of the dilepton production rate in the HIC, 
from Fig.~\ref{fig:Sigma3d} it is expected that the dilepton yield 
is enhanced when the medium created by the HIC goes through the red color region.



In Fig.~\ref{fig:SigmaComparison}, we finally show the behavior of $\sigma / T$ 
as a function of $\mu$ at $T = T_{\rm CP}$, i.e. along the dotted line 
in the left panel of Fig.~\ref{fig:Sigma3d} at $G_D = 0.7G_S$.
In the figure, the solid line represents the total contribution of $\sigma$, 
and the dashed (dotted) line is the contribution from the soft modes of the 2SC-PT (QCD-CP).
Since the QCD-CP is at $\mu_{\rm CP} \simeq 329~{\rm MeV}$,
the contribution of the QCD-CP is divergent there.
On the other hand, the contribution of the 2SC-PT
is divergent at $\mu \simeq 347~{\rm MeV}$ because 
the transition point of the 2SC-PT at $T = T_{\rm CP}$ exists there.
Moreover, one can see that the contribution of the 2SC-PT
is drastically decreasing around $\mu = \mu_{\rm CP}$.
This is explained as follows. In our approximations,
the denominators of the soft mode propagators are expanded in 
the direction of the energy at the origin of the energy/momentum plane of the soft mode.
The 2SC-PT soft mode exists in the region 
$|\omega + 2\mu| > \lambda(\bm{k}, 0)$ as shown in Eq.~\eqref{eq:ImQ_D},
and then, the approximations are available only when when $M < \mu$.
Additionally, at $M = \mu$, $\partial {\rm Im}Q^R(\bm{0}, \omega) / \partial \omega |_{\omega = 0} = 0$.
From these facts, the drastic decrease of $\sigma$ due to the 2SC soft modes can be understood.



Let us give the brief summary for the analysis of the transport coefficients.
In this chapter, the effects of the 2SC-PT and QCD-CP soft modes on 
the electric conductivity $\sigma$ and the associated relaxation time $\tau_\sigma$ 
have been investigated through the analysis of the photon self-energy 
including these modes in the two-flavor NJL model. 
We considered the low energy/momentum limit of the AL, MT, and DOS terms for the photon self-energy. 
These terms constitute the self-energy in a gauge-invariant manner 
including the effects of the soft modes at the mean-field level.
Through the analytic and numerical calculations, we have shown that the transport coefficients 
are enhanced near the 2SC-PT and QCD-CP with the power-like behavior owing to the existence 
of the soft modes near the respective phase transitions. 
Through the analytical analysis of the critical exponents of the transport coefficients,
it has been shown that the origin of divergences is due to the soft modes
and the difference in exponents comes from the different properties of the soft modes.
As described in Sec.~\ref{sec:DPR-Coeff}, the electric conductivity is related to 
the low energy and momentum behavior of the dilepton production rate (DPR)
through the photon self-energy or electric current-current correlator.
In the next Chapter, we will show the enhancement of the DPR due to the soft modes.


\begin{figure}[t]
\centering
\hspace{-1.5cm}
\includegraphics[keepaspectratio, scale=0.52]{Figures/SigmaComparison.pdf}
\caption
{Comparison of the contributions of $\sigma / T$
from the 2SC-PT and the QCD-CP soft modes at $T = T_{\rm CP}$.
The solid line represents the total contribution of $\sigma / T$, 
and the dashed, and dotted lines are the ones 
from the soft modes of the 2SC and the QCD-CP, respectively.}
\label{fig:SigmaComparison}
\end{figure}

\red{
% There are interesting extensions of the present study. 
% First, our formalism is not applicable to the 2SC phase.
% To investigate the behavior of the transport coefficients inside the 2SC phase~\cite{Jaikumar:2001jq},
% the formalism has to be extended to consider the effects of finite $\Delta$.
% Another interesting subject is to investigate the coupling between the soft mode of the QCD-CP 
% and the density fluctuations~\cite{Fujii:2003bz,Fujii:2004jt,Son:2004iv}. 
% It is known that the QCD-CP soft mode is a diffusive mode due to the coupling, 
% while this effect is not included in our formalism. 
% In the NJL model, this effect can be described by the vector interaction~\cite{Kitazawa:2001ft}. 
% Investigating its effects on the transport coefficients is another important extension of the present study.
% Finally, as discussed already, our analysis deals with the effects of the critical fluctuations at the mean-field level in the sense that their mutual interactions are not taken into account. Although this treatment enables a simple analysis, to realize a more quantitative analysis in the vicinity of the critical point the formalism should be extended to incorporate the non-linear effects.
% We also note that our analysis is not self-consistent in the sense that the effects of the soft modes are not incorporated into the thermodynamic potential nor quark propagator composing the soft modes. 
% Because of this inconsistency, we did not investigate the quark-number susceptibility $\chi$. Once $\chi$ is obtained, one can study the behavior of the diffusion coefficient $D=\sigma/\chi$ and the velocity of the shock $c_s=\cdots$ near the critical point.
% We leave these interesting analyses for the future study.
}

% \red{
% It is also important to pursue phenomenological consequences of our study in the HIC experiments. Since the electric conductivity is related to the DPR at low invariant-mass region, our result indicates that the DPR is enhanced near the QCD-CP and 2SC-PT~\cite{Nishimura:2022mku,Nishimura:2023not}.
% Although a distinguishment of these transitions would be difficult, recently it has been suggested in Ref.~\cite{Nishimura:2023oqn} that the DPR has a non-monotonic dependence on the collision energy $\sqrt{s_{_{NN}}}$ reflecting the fact that the conductivity is enhanced at two isolated regions as shown in Fig.~\ref{fig:sigma_3d}.
% It is interesting to make this argument quantitative further, which would be realized by incorporating other medium effects~\cite{Rapp:2009yu,Lattice,perturbation}.
% In the HIC, a direct analysis of electric conductivity would also be possible~\cite{exp-sigma}.
% To investigate the critical enhancement of these observables in the HIC, it is also important to describe the effects of the critical slowing down. 
% Whereas our formalism assumes thermalized system, to describe it the non-equilibirium effects should be included.
% }

\begin{comment}
In this paper, we have not considered the effect of the finite diquark condensate
$\Delta$, whose analysis would make it possible to investigate 
the behavior of the coefficients from below the transition line of the 2SC. 
It is necessary to introduce the vector coupling into our formalism, 
which changes the location of the boundary of the 2SC and the QCD-CP. 
Additionally, the property of the QCD-CP soft mode can be affected 
by that coupling through the mixing with the density fluctuation. 
Therefore, the study of the vector coupling leads to 
a deeper understanding of the critical effect on the transport property.
We would analyze the diffusion constant in our formalism to discuss the causality.
These studies should be dealt with in the future. 
Also, we need to consider the non-equilibrium effect, for example, the critical slowing down. 
This is one of the future tasks as well.

Recently, the study of electric conductivity through the observation of 
the ultra-low-energy dilepton production has been proposed in the heavy-ion collision experiments. 
Therefore, the divergences or enhancements of the conductivity that have been obtained 
in our study might provide an experimental signal for the CSC and QCD-CP, 
as well as the anomalous enhancement of the dilepton production rate shown in previous studies.
\end{comment}





